Status of kinematic cosmology with SN Ia: JLA, Pantheon and future constraints with LSST

In this work we derive state-of-the-art model-independent constraints on cosmology from SN Ia by measuring purely kinematical $\left( q,j \right)$ model parameters (where $q$ and $j$ are related to the first and second derivative of the Hubble parameter). For the JLA compilation of SN Ia an agreement within 2$\sigma$ of $\Lambda$CDM expectations is found, where best-fitting kinematical parameters are $q=-0.66 \pm 0.11$ and $j=0.41 ^{+0.32}_{-0.33}$. With $q=-0.73 \pm 0.13$ and $j=0.76 ^{+0.41}_{-0.43}$ the Pantheon sample shows even better agreement with the $\Lambda$CDM expectation of $j=1$ than JLA, hinting at less systematics and/or a higher number of SN Ia alleviating tensions. For the future we predict the precision achievable with SN Ia from the LSST deep survey as $\Delta q \sim 0.05$ and $\Delta j \sim 0.1$, which is systematics-limited and could lead to detect both deviations from $\Lambda$CDM (in $j$) or current expansion rates measured (in $q$). In comparison, for standard cosmological parameters we get $\Delta \Omega_\mathrm{m}=0.01$ and $\Delta w=0.07$ for LSST. Given the high number of SN Ia expected for LSST, kinematical parameters in up to 500 sky regions, each with their own individual Hubble diagram, can be constrained. For each region an individual precision at the 10s of percent level is within reach at current systematics-levels, comparable to present-day full-sky surveys. This will determine anisotropy in cosmic expansion, or the dark energy dipole, at the 10s of percent level at 10s of degree scales.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
